On the Rise and Fall of Simple Stupid Bugs: a Life-Cycle Analysis of SStuBs

Bug detection and prevention is one of the most important goals of software quality assurance. Nowadays, many of the major problems faced by developers can be detected or even fixed fully or partially with automatic tools. However, recent works explored that there exists a substantial amount of simple yet very annoying errors in code-bases, which are easy to fix, but hard to detect as they do not hinder the functionality of the given product in a major way. Programmers introduce such errors accidentally, mostly due to inattention. Using the ManySStuBs4J dataset, which contains many simple, stupid bugs, found in GitHub repositories written in the Java programming language, we investigated the history of such bugs. We were interested in properties such as: How long do such bugs stay unnoticed in code-bases? Whether they are typically fixed by the same developer who introduced them? Are they introduced with the addition of new code or caused more by careless modification of existing code? We found that most of such stupid bugs lurk in the code for a long time before they get removed. We noticed that the developer who made the mistake seems to find a solution faster, however less then half of SStuBs are fixed by the same person. We also examined PMD's performance when to came to flagging lines containing SStuBs, and found that similarly to SpotBugs, it is insufficient when it comes to finding these types of errors. Examining the life-cycle of such bugs allows us to better understand their nature and adjust our development processes and quality assurance methods to better support avoiding them.

==> abstract.tex <==
%The expected quality of software has had a steady increase ever since its very inception.
%Most of the major problems faced by developers are already detectable, or even preventable by fully, or partially automatic tools.
%One of the more difficult to detect issues are the ones, that do not hinder the functionality of the given product in a major way.
%Finding and fixing these is considered difficult and cumbersome.
%
%Our goal throughout the creation of this study was to create statistics in order to numerically back up the already widely accepted notion, when it comes to these kinds of bugs.
%In order to gather meaningful information about the issues in question, we needed not only the way and place they were fixed at, which we got from the ManySStuBs4J dataset, but also their source.
%Examining the life-cycle of these bugs allowed us to come to a greater understanding, when it comes to the challenge of detecting and handling them.
%We found that on average it takes a considerable amount of time to get rid of these issues, and that most of them do not get fixed by the developer who introduced them.

Bug detection and prevention is one of the most important goals of software quality assurance.
Nowadays, lots of the major problems faced by developers can be detected or even fixed fully or partially with automatic tools.
However, recent works explored that there exists a substantial amount of simple, yet very annoying errors in code-bases, which are easy to fix, but hard to detect as they do not hinder the functionality of the given product in a major way.
Programmers introduce such errors accidentally mostly due to inattention.

Using the ManySStuBs4J dataset, which contains a large number of such simple, stupid bugs, we investigated the history of such bugs.
We were interested in properties like, how long do such bugs stay unnoticed in code-bases, whether they are typically fixed by the same developer who introduced them, or are they introduced with the addition of new code or caused more by careless modification of existing code?
We found that most of such stupid bugs lurk in the code for a long time before they get removed, and that most of them are not fixed by the developer who introduced them.
Examining the life-cycle of such bugs allows us to better understand their nature and adjust our development processes and quality assurance methods to better support avoiding them.
